Security Properties for Open-Source Hardware Designs

The hardware security community relies on databases of known vulnerabilities and open-source designs to develop formal verification methods for identifying hardware security flaws. While there are plenty of open-source designs and verification tools, there is a gap in open-source properties addressing these flaws, making it difficult to reproduce prior work and slowing research. This paper aims to bridge that gap. We provide SystemVerilog Assertions for four common designs: OR1200, Hack@DAC 2018's buggy PULPissimo SoC, Hack@DAC 2019's CVA6, and Hack@DAC 2021's buggy OpenPiton SoCs. The properties are organized by design and tagged with details about the security flaws and the implicated CWE. To encourage more property reporting, we describe the methodology we use when crafting properties.

==> intro_ideas.tex <==
\begin{itemize}[noitemsep]
\item Hard to reproduce results when don't have assertions.
\item Different assertions for different tools and designs.
\item Discrepancies we resolved.
\item Discrepancies between our results and other results.
\item Don't know exact version of tool or design.
\item Difficulties/limitations of writing properties - from known bugs.
\item The quality of the properties matters. Can we find bugs using commercial
  tools that other papers reported as not-found with the same tools simply by
  writing better properties?
  \end{itemize}

\jsr{Draft of the intro section, full paragraphs to be added}
General info about the field
\begin{itemize}[noitemsep]
\item Hardware(verilog, rtl representations of hardware)
\item hardware vulnerabilities
\item current research (how is the problem of hardware security being addressed)
\end{itemize}
Formal verification
\begin{itemize}[noitemsep]
\item short description
\item tools (Manual inspection, Simulation, Model Checking (JG), Symbolic execution (Sylvia))
\item SVA to verify properties (assert, cover)
\end{itemize} 
Goals
\begin{itemize}[noitemsep]
\item paper contributions
\end{itemize}

\subsection{First Framing Possibility}
\cks{Some rough thoughts on framing the paper}
This paper makes two contributions. First, we demonstrate that the properties
used in the formal verification of hardware designs are not being adequately
reported in the literature. We conduct a methodical review of the literature and
find that XX\% of the time, formally stated properties used during the
evaluation of new verification tools and techniques are not reported. We
contrast this with the reporting rate for other aspects of the evaluation set-up,
such as the open-source designs used (reported XX\% of the time) and bugs found (XX\%).

% our central hypothesis
In the second contribution, we demonstrate that without adequately reporting on
the properties used during formal verification, we cannot fairly judge the
strengths and limitations of any given formal verification tool. 

% three supporting arguments
\cks{These are all hypotheses at this point. If we like this framing, we can use these to guide
  the research. We will have to show that the research bears these out. If it
  does not, we'll need to reconsider our framing.}
\paragraph*{\#1} We cannot fairly judge the efficacy of new formal verification tools without
also considering the properties used during the evaluation. 
\begin{itemize}[noitemsep]
  \item We show that some
papers' reported results comparing their tool to existing state of the art and
commercial tools under-report the efficacy of the existing tool.
\item We posit that
this is because the properties developed to maximize efficacy of their tool does
not necessarily maximize the efficacy of the existing tools. We make this case
next.
  \item Our objective is not to denigrate those papers -- they were evaluating a tool,
not a set of properties. 
\item We compare only to commercial tools because we found the majority of state
  of the art tools reported in the literature are not open-source (a separate
  problem from that of reporting properties).
\end{itemize}

\paragraph*{\#2} Properties written for use with one tool are not necessarily
directly useful/optimal for use with another tool.
\begin{itemize}[noitemsep]
  \item We show that properties written for Cadence JasperGold do not produce the best results for Symbiyosys or
Sylvia (or vice-versa). Rather, rewriting the property to better leverage the
underlying technology of the tool produces better results in terms of efficacy
(or performance)
\item Just as properties written for one design need to be rewritten to be
  useful with another design~\cite{zhang2020transys}, so too properties written
  for use with one tool need to be rewritten for use with a second tool.
\item \cks{Not at all clear at this stage whether this hypothesis will bear out!}
\end{itemize}

\paragraph*{\#3} Reporting only bugs found/not found and tools/platforms/designs
used is not enough to make the work reproducible. The properties used in the
evaluation must also be reported.
\begin{itemize}[noitemsep]
\item We show there are many degrees of freedom that
  exist when only a bug description is given.
\item The result is that two different
tool creators may write two very different properties for the same bug
description.
\item Given the first two findings, this means that any reported results
claiming to compare a new tool to prior tools is unreliable at best.
\item We describe the challenges of writing properties
given only bug descriptions. 
\end{itemize}

\subsection{Second Framing Possibility}


==> lit_review.tex <==
\section{Literature Review}
\label{sec:lit-review}

% Methodology
Our literature review proceeded in two phases: collecting papers to consider for
inclusion in the literature review and deciding whether to include the paper.

\subsection{Phase 1: Collecting Papers}
We started with three recent papers we knew from our prior work to be relevant to 
our investigation of the use of security properties with formal verification
tools and that are well cited. These papers 
were ``HardFails: Insights into software-exploitable hardware bugs'' by Dessouky et al.~\cite
{dessouky2019fails}, ``RTL-ConTest: Concolic Testing on RTL for Detecting Security Vulnerabilities'' 
by Meng et al.~\cite{meng2021rtl}, and ``End-to-End Automated Exploit Generation for Validating the 
Security of Processor Designs'' by Zhang et al.~\cite{zhang2018end}. We put
these three papers in our To Include stack, and for each one we collected
all the papers in its References section and put those papers in our To Consider
stack, as long as the paper was published no earlier than 2015.

We then used \url{scholar.google.com} to find the list of papers citing each of
the three papers in our To Include stack. We added these papers to our To
Consider stack as well.

\subsection{Phase 2: Deciding Whether to Include a Paper}
For every paper in our To Consider stack, we used the following three steps to
decide whether to add the paper to our To Include stack and include the paper in
our literature review.

First, if the paper's title made it clear the paper was irrelevant to our review, we 
discarded it. In the cases where the paper came from the References section of
another paper, we also considered the citing paper's description to identify
papers that were clearly irrelevant. %% \kar{is there an example of one we were able to discard based
%% on this criteria? Plug in here.}
Second, for all remaining papers, we read the abstract and kept the paper in our stack 
if the paper was related to formal verification methods for hardware designs or the use or 
development of security properties for formal verification of hardware designs. Third, for all 
remaining papers, we read the paper and deemed the paper relevant if it presents formal verification results involving property-checking or finding assertion violations, 
or if the paper presents a new automated security property generation tool or
framework. These papers got added to the To Include stack.

Every time a new paper was added to the To Include stack, we repeated phase 1,
collecting the papers it cites and the papers that cite it.
We iterated over these two phases until we reached a fixpoint in which we found
no new papers in the collecting phase.


%% % Just re-orged this text a little in the above. Kept the original here in
%% case I messed up too badly.

%% To collect papers, we started with three recent papers we knew from our prior work to be relevant to 
%% our investigation of the use of security properties with formal verification tools. These papers 
%% were ``HardFails: Insights into software-exploitable hardware bugs'' by Dessouky et al.~\cite
%% {dessouky2019fails}, ``RTL-ConTest: Concolic Testing on RTL for Detecting Security Vulnerabilities'' 
%% by Meng et al.~\cite{meng2021rtl}, and ``End-to-End Automated Exploit Generation for Validating the 
%% Security of Processor Designs'' by Zhang et al.~\cite{zhang2018end}. For each of these papers, we 
%% determined which papers included in their References sections to include in our literature 
%% review. The process for determining the inclusion of cited papers proceeded in three stages.

%% First, if the containing paper's 
%% description or the cited paper's title made it clear the paper was irrelevant to our review, we 
%% discarded it. For example, \kar{is there an example of one we were able to discard based
%% on this criteria? Plug in here.}
%% Second, for all remaining papers, we read the abstract and kept the paper in our stack 
%% if the paper was related to formal verification methods for hardware designs or the use or 
%% development of security properties for formal verification of hardware designs. Third, for all 
%% remaining papers, we read the paper and deemed the paper ``relevant'' if it presents some
%% formal verification results involving property-checking or finding assertion violations, 
%% or if the paper presents a new automated security property generation tool or framework.

%% We then repeated this process in reverse, collecting papers that cited the original three papers of interest.
%% We used \url{scholar.google.com} to find the list of papers citing our 
%% original three. For each paper found, we repeated the same process as above, requiring that each
%% included paper was published post-2014.

%% Finally, we repeated this entire process, for each new paper we
%% deemed relevant. We analyzed the papers in each References section and the 
%% papers that cited each one. We continued to iterate until we reached a fixpoint and found no new papers. 

\subsection{Papers Included}
% Numbers for Literature Review
In total, we read 114 papers, and deemed 28 relevant to our question. Of these
papers, 20 performed 
formal verification and reported their results in the evaluation section of their work; 7 papers 
presented a novel security property generation tool or framework; 1 paper presented a security 
property generation framework and reported the results of using the generated
properties for formal verification in their evaluation. The papers spanned the nine years from 2015 to 2024, and were 
published in a range of venues spanning conferences in hardware architecture and design, CAD, and 
security (e.g., MICRO, ICCAD, DAC, Oakland), journals (e.g., IEEE Transactions
on Computer-Aided Design of Integrated Circuits and Systems), preprints, and
theses. The full set of papers we included are listed in our repository here: \url{https://anonymous.4open. science/r/verification-benchmarks-C1C5/}.

For each of the 28 papers, we 
took note of how security properties factored into their 
research. If a paper reported the results of formal verification of hardware designs, we recorded 
the designs and formal analysis tools used and identified whether or not the paper reports the 
natural-language security properties, formally stated assertions, and bugs involved in their verification process.

%% \subsection*{Methodology}
%% During our literature review, we examined over 100 hardware security papers. To collect papers, we 
%% started with a small set of papers we knew to be relevant to our research question on formal 
%% verification and security properties from prior work. Then, we combed through these papers’ cited 
%% works and the works citing these papers. In the review process, we looked specifically for papers 
%% relating to formal verification methods and security properties for formal verification. For papers 
%% relevant to our research question, we took note of how security properties factored into their 
%% research. If a paper reported the results of formal verification of hardware designs, we recorded 
%% the designs and formal analysis tools used and identified whether or not the paper reports the 
%% security properties, assertions, and bugs involved in their verification process.

% Analysis
Of the 21 papers that performed formal verification on hardware designs, we
identified three main 
categories of works. The first category includes papers that introduce a novel formal verification 
technique, tool, or methodology. These papers present their methodology and implementation first. 
Then, in the evaluation, they provide the results of using their tool for the formal verification of 
benchmark hardware designs. Some of these papers compared the verification results of their novel 
tool to the results of existing tools. We placed nine papers into this category
(\cite{meng2021rtl,zhang2018end,hicks2015specs,ryan2023sylvia,ryan2023countering,meng2023ensuring,fang2023wasim,7927266,lyu2020automated}). 

The next category includes papers that introduce frameworks that use existing 
formal verification tools rather than presenting a novel tool. These papers present 
novel frameworks for threat modeling, formal verification, and/or 
exploit generation. These papers used existing industry-standard formal verification tools,
such as Cadence's Jasper Formal Path Verification (FPV), OneSpin 360 Design Verification (DV) or 
Questa Formal Verification, as a component within the larger framework
they were presenting. Ten papers fell into this category, including the
paper that did both formal verification and property
generation~\cite{dipu2023agile,mehmedagic2023design,muller2021formal,anton2023fault,rajendran2023hunter,solem2023applying,rahmani2022unique,rajendran2024exploring,7308670,8587741}.

%%  includes papers that 
%% present novel techniques for automated property generation and then use existing formal verification 
%% tools to verify the properties generated by their tool. It 

The third category includes papers that provide an overview of hardware security 
methods. We found two papers that review hardware security methods and perform formal verification 
to evaluate that method of hardware security validation~\cite{dessouky2019fails,9000170}. These papers used the industry-standard 
commercial tool JasperGold FPV to evaluate security properties 
on benchmark designs and evaluate the efficacy and challenges of formal verification as a hardware 
design security technique.

The eight papers that present methods for property generation used a variety of
techniques. The most recent papers explored using large language model (LLM)
code generation to generate RTL properties~\cite{paria2023divas,kande2023llm,meng2023unlocking}.  Other techniques include cross-design property translation, mining
properties from design behavior, and using CWE descriptions to generate properties~\cite{zhang2020transys,dipu2023agile,deutschbein2021isadora,deutschbein2020evaluating,deutschbein2021mining}.

%% By prompting the 
%% LLMs with information like hardware design specifications, CWEs, or natural language property 
%% descriptions, researchers have been able to generate useful RTL-level assertions for hardware 
%% designs.

%% While manual property writing can be challenging and imperfect for the reasons discussed above, 
%% automating the property generation process has been a popular focus of research in recent years. 
%% Through our literature review, we encountered numerous papers introducing new tools and techniques 
%% for automatically generating hardware security properties. Some novel techniques for automated 
%% property generation include large language model (LLM) code generation, cross-design translation, 
%% specification mining, and Common Weakness Enumeration (CWE) mining.

%% %% In response to the challenges associated with manual property writing, automatic property generation 
%% %% has become an active area of research. Property generation tools aim to analyze hardware designs 
%% %% and/or design specifications and produce expressive properties that capture desired behavior. 
%% %% This line of work is discussed more in section X. 

%% As LLMs have been increasingly used for code generation, hardware security researchers have begun to 
%% explore the powerful AI tools' abilities to write hardware security properties. By prompting the 
%% LLMs with information like hardware design specifications, CWEs, or natural language property 
%% descriptions, researchers have been able to generate useful RTL-level assertions for hardware 
%% designs. Other techniques include mining RTL-level assertions directly from design specifications, 
%% CWEs,  or existing assertions written for different designs. All of these techniques seek to 
%% alleviate the challenges of manual property writing.

\subsection{Results}
For each paper performing formal verification, we examined how they reported 
the properties used in their evaluations. Specifically, we asked three 
questions about each paper:
\begin{enumerate}
  \item Does the paper describe the high-level (natural language) security properties which they 
  are seeking to verify?
  \item If the research uses an assertion-based verification tool, does the paper
  provide the assertions used in the verification process?
  \item Does the paper report the design bugs they found using their tool 
  or framework?
\end{enumerate}

In answering these questions our goal is to highlight the need for formally stated RTL assertions, 
rather than to call out prior work that does not provide these assertions. We provide only the
summary counts of papers answering each question and do not name the individual
papers.

Considering question 1, we found that 14 of the 21 papers performing formal verification, described 
the high-level security properties they were verifying and 7 did not.

Question 2 is relevant only for papers performing an assertion-based
verification tool. Of the
21 papers presenting formal verification techniques, 18 fell into this category. Of these 18, only 4
papers provided all of the assertions they used during verification. Five of the
18 papers
provided some of the assertions they used. However, 4 of those 5 provided only one or two example assertions. The fifth paper was the one paper 
which both performed automated property generation and formal verification. 
This paper provided 10 of the most relevant assertions out of the thousands 
generated during the evaluation of their property generation tool.
Nine of the 18 
papers using assertion-based verification did not provide any of the assertions 
used in their evaluation.

Considering question 3, we found that 18 of the 21 papers performing formal verification discussed the design bugs they 
found with their tool or framework. The other two papers presented their 
results strictly in terms of time and memory needed to trigger assertion 
violations.

For the eight papers presenting automated security property generation techniques, 
we asked two questions:
\begin{enumerate}
  \item Does the paper describe the high-level security properties the tool 
  generated?
  \item Does the paper provide the RTL-level assertions the tool generated?
\end{enumerate}

Considering question 1, we found that all of the eight papers generating security properties included a 
high-level discussion of all the security properties generated by their tool. 
Considering question 2, we found that only one paper provided all of the assertions
generated by their tool. Six papers provided some but not all of the 
generated assertions. One paper only focused on generating security properties
at a higher abstraction level than RTL assertions. Most of the papers that 
provided some but not all assertions produced hundreds to thousands
of assertions with their framework and included a small handful of example assertions hand-chosen from 
the larger body of assertions.

\subsection{Literature Review Observations}
Comparing the reporting rates of properties to other components of the
evaluation, we find a difference. The open-source designs used during
formal verification were reported in 17 of the 21 papers and the bugs found
during formal verification were reported in 19 of the 21 papers.

We found that thesis papers we examined during 
the literature review tended to include more detailed and complete reporting of properties than 
conference-style papers. This may be because thesis papers do not have the same page count 
limitations that conference papers do. It may also be that authors of conference
papers underestimate the importance of the formally stated assertions for reproducibility.

Going into the literature review, we expected to find that papers performing
formal verification require formally stated assertions for their evaluation,
which is what we found. What was unexpected, though, was that many papers
presenting a technique for generating properties also require formally stated
assertions for their evaluation. For example, the paper that presented a technique for automatically translating
properties written for one design to make them useful for a second design
required a starting set of properties written for the first design to try to
translate for a second design~\cite{zhang2020transys}. As a second example, the
technique used in one of the papers investigating LLMs for assertion generation
involved first manually writing ten benchmarks, which was a snippet of buggy code
and natural-language description of the desired property, then manually writing
the SVA property to be used as a point of comparison when evaluating the
generated properties~\cite{kande2023llm}. The properties we provide here will
support larger, more comprehensive evaluations in both of these areas.

